A systematic mapping study on cross-project defect prediction

Cross-Project-Defect Prediction as a sub-topic of defect prediction in general has become a popular topic in research. In this article, we present a systematic mapping study with the focus on CPDP, for which we found 50 publications. We summarize the approaches presented by each publication and discuss the case study setups and results. We discovered a great amount of heterogeneity in the way case studies are conducted, because of differences in the data sets, classifiers, performance metrics, and baseline comparisons used. Due to this, we could not compare the results of our review on a qualitative basis, i.e., determine which approaches perform best for CPDP.

==> abstract.tex <==
% for Computer Society papers, we must declare the abstract and index terms
% PRIOR to the title within the \IEEEcompsoctitleabstractindextext IEEEtran
% command as these need to go into the title area created by \maketitle.
\IEEEcompsoctitleabstractindextext{%
\begin{abstract}
%\boldmath
\acf{CPDP} as a sub-topic of defect prediction in general has become a popular
topic in research. In this article, we present a systematic mapping study
with the focus on \ac{CPDP}, for which we found 50 publications. We summarize
the approaches presented by each publication and discuss the case study setups
and results. We discovered a great amount of heterogeneity in the way case
studies are conducted, because of differences in the data sets, classifiers,
performance metrics, and baseline comparisons used. Due to this, we could not
compare the results of our review on a qualitative basis, i.e., determine which
approaches perform best for \ac{CPDP}. Instead, we propose guidelines for how
future case studies on \ac{CPDP} should be conducted in order to ensure
comparabilty between publications. 
\end{abstract}
% IEEEtran.cls defaults to using nonbold math in the Abstract.
% This preserves the distinction between vectors and scalars. However,
% if the journal you are submitting to favors bold math in the abstract,
% then you can use LaTeX's standard command \boldmath at the very start
% of the abstract to achieve this. Many IEEE journals frown on math
% in the abstract anyway. In particular, the Computer Society does
% not want either math or citations to appear in the abstract.

% Note that keywords are not normally used for peer review papers.
\begin{keywords}
cross-project defect prediction, literature review, mapping study
\end{keywords}}
